Constraining Progenitors of Observed LMXBs Using CARB Magnetic Braking

We present a new method for constraining the mass transfer evolution of low mass X-ray binaries (LMXBs) - a reverse population synthesis technique. This is done using the detailed 1D stellar evolution code MESA (Modules for Experiments in Stellar Astrophysics) to evolve a high-resolution grid of binary systems spanning a comprehensive range of initial donor masses and orbital periods. We use the recently developed Convection And Rotation Boosted (CARB) magnetic braking scheme. The CARB magnetic braking scheme is the only magnetic braking prescription capable of reproducing an entire sample of well studied persistent LMXBs -- those with their mass ratios, periods and mass transfer rates that have been observationally determined. Using the reverse population synthesis technique, where we follow any simulated system that successfully reproduces an observed LMXB backwards, we have constrained possible progenitors for each observed well-studied persistent LMXB. We also determined that the minimum number of LMXB formations in the Milky Way is 1500 per Gyr if we exclude Cyg X-2. For Cyg X-2, the most likely formation rate is 9000 LMXB per Gyr. The technique we describe can be applied to any observed LMXB with well-constrained mass ratios, period and mass transfer rate. With the upcoming GAIA DR3 containing information on binary systems, this technique can be applied to the data release to search for progenitors of observed persistent LMXBs.

==> rand_table.tex <==
\begin{table}
\caption{\textbf{Calculated Rates}}
\centering
\begin{tabular}{l | ll}
% \hline

Property            & With Cyg X-2 & Without Cyg X-2 \\
\hline

Average             &  125913      & 8766   \\
Min                 &  2827        & 1452   \\
Max                 &  1386667     & 101017 \\

\hline

\end{tabular}
\label{table:rand_table}
\begin{flushleft}
\footnotesize
\textbf{Notes.} This table shows the average, minimum and maximum calculated formation rates when we randomly select a progenitor for our observed LMXBs.
\end{flushleft}
\end{table}
